SafeRoute: Adaptive Model Selection for Efficient and Accurate Safety Guardrails in Large Language Models

Deploying large language models (LLMs) in real-world applications requires robust safety guard models to detect and block harmful user prompts. While large safety guard models achieve strong performance, their computational cost is substantial. To mitigate this, smaller distilled models are used, but they often underperform on "hard" examples where the larger model provides accurate predictions. We observe that many inputs can be reliably handled by the smaller model, while only a small fraction require the larger model's capacity. Motivated by this, we propose SafeRoute, a binary router that distinguishes hard examples from easy ones. Our method selectively applies the larger safety guard model to the data that the router considers hard, improving efficiency while maintaining accuracy compared to solely using the larger safety guard model. Experimental results on multiple benchmark datasets demonstrate that our adaptive model selection significantly enhances the trade-off between computational cost and safety performance, outperforming relevant baselines.

==> captions/fig_aug_ablation.tex <==
\begin{figure}[t]
\medskip
\centering
\includegraphics[width=0.8\columnwidth]{images/aug_ablation.pdf}
\vspace{-0.5em}
\caption{Average F1 score as a function of the number paraphrases for each data point.}
\label{fig:aug_ablation}
\vspace{-0.15in}
\end{figure}

==> captions/fig_three.tex <==
\begin{figure*}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{images/jailbreaktype.pdf}
        \captionof{figure}{Number of larger model selections for each jailbreak attack on the Harmbench dataset.}
        \label{fig:jailbreaktype}
    \end{minipage}
    \hfill
    \hspace{0.001in}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \resizebox{0.95\columnwidth}{!}{\begin{tabular}{lc}
    \toprule
    \textbf{Method}     & \textbf{Avg. F1} \\
    \midrule
    \rowcolor{rowgray}
    \texttt{ModernBERT}         & 0.1001  \\
    \midrule
    Layer 2 & 0.1039 \\
    \rowcolor{rowgray}
    Layer 4 & 0.0686\\
    Layer 6 & 0.0462 \\
    \rowcolor{rowgray}
    Layer 8  &0.0375\\
    Layer 10 &0.3423 \\
    \rowcolor{rowgray}
    Layer 12 & 0.3940 \\
    Layer 14 & 0.4320 \\
    \midrule
    \rowcolor{rowgray}
    w/o Paraphrasing (layer 16) & 0.4424 \\
    \midrule
    \textbf{Full model} (layer 16) & \textbf{0.4964} \\
    \bottomrule
    \end{tabular}
    }
    \captionof{table}{We ablate each component of our router and report average routing F1 score across six datasets.}
    \label{tab:ablation}
    \end{minipage}    
    \hfill
    \hspace{0.001in}
    \begin{minipage}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=0.95\textwidth]{images/aug_ablation.pdf}
\caption{Average routing F1 score across six datasets vs. the number of paraphrases per data point.}
\label{fig:aug_ablation}
\end{minipage}
\end{figure*}

==> captions/tab_ablation.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.65\columnwidth}{!}{\begin{tabular}{lc}
    \toprule
    \textbf{Method}     & \textbf{Avg. F1} \\
    \midrule
    \texttt{ModernBERT}         & 0.1001  \\
    \midrule
    Layer 2 & 0.1039 \\
    Layer 4 & 0.0686\\
    Layer 6 & 0.0462 \\
    Layer 8  &0.0375\\
    Layer 10 &0.3423 \\
    Layer 12 & 0.3940 \\
    Layer 14 & 0.4320 \\
    \midrule
    w/o Paraphrasing (layer 16) & 0.4424 \\
    \midrule
    \textbf{Full model} (layer 16) & \textbf{0.4964} \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-0.5em}
    \caption{We ablate each component of our router and report average F1 score across 6 benchmark datasets.}
    \label{tab:ablation}
    \vspace{-0.15in}
\end{table}

==> captions/tab_main_results.tex <==
\begin{table*}[t]
\caption{We run experiments five times with different random seeds and report the average F1 and AUPRC scores. The best results are bolded and the second-best are underlined.} 
\vspace{-1em}
\label{tab:main_results}
\resizebox{1.0\textwidth}{!}{

\begin{tabular}{lcccccccccccccc}

\toprule

& \multicolumn{2}{c}{\textbf{WildGuardMix-p}}
& \multicolumn{2}{c}{\textbf{Toxic-Chat}}
& \multicolumn{2}{c}{\textbf{OAI}}
& \multicolumn{2}{c}{\textbf{WildGuardMix}}
& \multicolumn{2}{c}{\textbf{XSTest}}
& \multicolumn{2}{c}{\textbf{HarmBench}}
& \multicolumn{2}{c}{\textbf{Average}} \\

\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
\cmidrule(lr){12-13}
\cmidrule(lr){14-15}

\textbf{Model}
& F1 & AUPRC
& F1 & AUPRC
& F1 & AUPRC
& F1 & AUPRC
& F1 & AUPRC
& F1 & AUPRC 
& F1 & AUPRC \\

\midrule
Entropy
&  & 
&  & 
&  & 
&  & 
&  &  
&  &  \\
+TS 
& 0.7904 & 0.6908 
& 0.7045 & 0.5704 
& 0.9041 & 0.8482 
& 0.8490 & 0.7780 
& 0.6781 & 0.7733 
& 0.7852 & 0.7321 \\
+CC 
& 0.7575 & 0.6331 
& 0.7276 & 0.5907 
& 0.8919 & 0.8247 
& 0.8345 & 0.7503 
& 0.6736 & 0.7719 
& 0.7770 & 0.7141 \\
+BC 
& 0.7612 & 0.6437 
& 0.7134 & 0.5793 
& 0.8919 & 0.8247 
& 0.8441 & 0.7671 
& 0.6614 & 0.7679 
& 0.7744 & 0.7165 \\
\midrule
Ours
&  & 
&  & 
&  & 
&  & 
&  &  
&  &  \\
\bottomrule
\end{tabular}
\vspace{-0.15in}

}
\end{table*}

